STaRFormer: Semi-Supervised Task-Informed Representation Learning via Dynamic Attention-Based Regional Masking for Sequential Data

Understanding user intent is essential for situational and context-aware decision-making. Motivated by a real-world scenario, this work addresses intent predictions of smart device users in the vicinity of vehicles by modeling sequential spatiotemporal data. However, in real-world scenarios, environmental factors and sensor limitations can result in non-stationary and irregularly sampled data, posing significant challenges. To address these issues, we propose STaRFormer, a Transformer-based approach that can serve as a universal framework for sequential modeling. STaRFormer utilizes a new dynamic attention-based regional masking scheme combined with a novel semi-supervised contrastive learning paradigm to enhance task-specific latent representations. Comprehensive experiments on 56 datasets varying in types (including non-stationary and irregularly sampled), tasks, domains, sequence lengths, training samples, and applications demonstrate the efficacy of STaRFormer, achieving notable improvements over state-of-the-art approaches.

==> content/12_figures/1_cl-approach.tex <==
\begin{figure}[!ht]
    \vskip 0.1in
    \centering
    \resizebox{.9\linewidth}{!}{%
        \input{content/10_drawings/1_cl-approach}
    }
    \caption{STaRFormer's \gls{cl} approach: The masking, $g$, generates two correlated views. The encoder, $f$, is trained to maximize the trade-off between batch- and class-wise agreement of the latent embeddings $\mathbf{Z}$ and $\tilde{\mathbf{Z}}$ while training for a downstream task.}
    \label{fig:cl-schematic-starformer}
    %\vspace{-0.7cm}
    \vskip -0.1in
\end{figure}

==> content/13_tables/ablation_results.tex/2_contrastive.tex <==
\adjustbox{max width=1\linewidth}{
    \begin{tabular}{l|c c | c c | c c c c}
    \toprule
    \toprule
     \multirow{2}{*}{CL Method}& \multicolumn{2}{|c|}{\gls{DKT} ($ \lambda_{\mathrm{CL}} \approx 0.796$)} & \multicolumn{2}{|c|}{\gls{GL} ($\lambda_{\mathrm{CL}} \approx 0.773$)} & \multicolumn{4}{|c}{\gls{PAM} ($\lambda_{\mathrm{CL}} \approx 0.567$)} \\
     & Acc & F$_{0.5}$ & Acc & F$_{0.5}$ & Acc & Precision & Recall & F$_{1}$ \\  
    \midrule
    semi-supervised & $\textbf{85.2} \pm 0.3$ & $\textbf{85.2} \pm 0.3$ 
    % & 90.5 $\pm 0.7$ & 88.6 $\pm 0.3$ 
    & $90.4 \pm 1.6$& $88.3 \pm 1.9$
    & $\textbf{97.6} \pm 0.9$ & $97.3 \pm 0.4$ & $\textbf{97.6} \pm 0.3$ & $\underline{97.4} \pm 0.3$ \\
    \midrule
    w/o self-supervised & $84.8 \pm 0.2$ & $84.8 \pm 0.2$ 
    % & 89.6 $\pm 0.6$ & 88.1 $\pm 0.6$ 
    & $90.0	\pm 1.4$ & $87.7 \pm 1.5$
    &  $96.3 \pm 1.9$ & $97.0 \pm 0.7$ & $96.9 \pm 0.5$ & $97.3 \pm 0.8$ \\
    
    w/o supervised & $84.8 \pm 0.1$ & $84.7 \pm 0.2$ 
    % & 90.2 $\pm 1.0$ & 88.4 $\pm 0.8$ 
    & $89.5 \pm 1.6$& $87.7 \pm 1.4$
    & $96.5 \pm 1.6$ &  $\underline{97.5} \pm 0.3$ &  $\underline{97.4} \pm 0.5$ &  $ \underline{97.4} \pm 0.3$ \\ 
    
    \midrule
    semi-supervised, 
    $\lambda_{\mathrm{CL}} = 0.1$ & $84.8 \pm 0.1$ & $84.6 \pm 0.4$ 
    % & $89.4 \pm 0.7$ & $87.7 \pm 0.4$ 
    & $90.0\pm 1.8$& $87.9\pm 2.1$
    & $96.8 \pm 1.2$ &$96.9 \pm 0.2$ &$97.3 \pm 0.3$ &$97.1 \pm 0.1$ \\
       
    semi-supervised, 
    $\lambda_{\mathrm{CL}} = 1$ & 
    $\underline{85.1} \pm 0.2$ & $\underline{85.1} \pm 0.2$ 
    %& $90.2 \pm 0.7$ & $88.5 \pm 0.5$ 
    & $90.2 \pm	1.3$& $88.0 \pm	1.5$
    & $\underline{97.2} \pm 0.7$ & $97.4 \pm 0.3$ & $97.2 \pm 0.7$ & $97.3 \pm 0.4$\\

    semi-supervised, 
    $\lambda_{\mathrm{CL}} = 5$ & $84.9 \pm 0.2$ & $84.9 \pm 0.2$ 
    % & $91.0 \pm 0.3$ & $89.7 \pm 0.3$
    & $\textbf{90.8} \pm 1.3$& $\textbf{88.7} \pm 1.6$
    & $96.7 \pm 2.3$ & $\underline{97.5} \pm 1.2$ &$97.0 \pm 1.7$ &$97.2 \pm 1.5$ \\

    semi-supervised, $\lambda_{\mathrm{CL}} = 10$ & $84.6 \pm 0.3$ &  $84.6 \pm 0.3$ 
    %& $90.6 \pm 0.4$ & $89.1 \pm 0.4$
    & $\underline{90.6} \pm 1.0$ & $\underline{88.5} \pm 1.3$
    & $97.0 \pm 1.6$ & $\textbf{97.7} \pm 0.7$ & $\textbf{97.6} \pm 0.7$ & $\textbf{97.6} \pm 0.7$ \\
    \bottomrule
    \bottomrule
    \end{tabular}
}


==> content/13_tables/ablation_results.tex/3_masking.tex <==
\adjustbox{max width=1\textwidth}{
    \begin{tabular}{ c | c c | c c | c c c c } 
        \toprule
        \toprule
         & \multicolumn{2}{c|}{\gls{DKT} $( \varphi\approx0.427, \zeta=0.2 )$} & \multicolumn{2}{c|}{\gls{GL} $( \varphi\approx0.472, \zeta=0.3 )$} & \multicolumn{4}{c}{\gls{PAM} $( \varphi\approx0.207, \zeta=0.3 )$} \\ %\cline{3-10}
        $\gamma$ & Accuracy & F$_{0.5}$ & Accuracy & F$_{0.5}$ & Accuracy & Precision & Recall & F$_{1}$  \\ 
        \midrule
        0.00  & 
        $85.0 \pm 0.2$ &$85.0 \pm 0.2$ & 
        $89.8 \pm 1.9$ & $87.9 \pm 1.8$ &
        $97.0 \pm 0.7$ & $\underline{97.4} \pm 0.2$ & $97.3 \pm 0.6$ & $97.3 \pm 0.3$ \\
        0.05 & 
        $85.0 \pm 0.3$ & $84.8 \pm 0.3$ & 
        $\textbf{90.4} \pm 1.6$ & $\underline{88.3} \pm 1.9$ & 
        $94.9 \pm 2.5$ & $96.5 \pm 0.6$ & $96.6 \pm 0.5$ & $96.5 \pm 0.4$ \\
        0.10 & 
        $84.9 \pm 0.3$ & $84.9 \pm 0.2$ &
        $\underline{90.3} \pm 1.2$ & $88.2 \pm 1.3$ &
        $\textbf{97.6} \pm 0.9$ & $97.3 \pm 0.4$ & $\textbf{97.6} \pm 0.3$ & $\underline{97.4} \pm 0.3$ \\
        0.15 & 
        $85.0 \pm 0.2$ & $85.0 \pm 0.2$ &
        $\underline{90.3} \pm 1.5$ & $88.2 \pm 1.7$ &
        $\underline{97.1} \pm 1.1$ & $\textbf{97.5} \pm 0.6$ & $\underline{97.5} \pm 1.0$ & $\textbf{97.5} \pm 0.8$ \\
        0.20 &
        $\underline{85.1} \pm 0.1$ & $\underline{85.1} \pm 0.1$ &
        $90.1 \pm 1.1$ & $87.9 \pm 1.0$ &
        $96.2 \pm 0.8$ & $96.7 \pm 0.5$ & $96.6 \pm 0.6$ & $96.6 \pm 0.4$ \\
        0.25 & 
        $\textbf{85.2} \pm 0.3$ & $\textbf{85.2} \pm 0.3$ &
        $90.1 \pm 1.6$& $\textbf{88.4} \pm 1.4$ &
        $96.3 \pm 0.9$ & $96.9 \pm 0.7$ & $96.5 \pm 0.6$ & $96.7 \pm 0.5$ \\
        0.30 & 
        $85.0 \pm 0.1$ & $85.0 \pm 0.1$ & 
        $\underline{90.3} \pm 1.3$ & $88.2 \pm 1.4$ &
        $96.3 \pm 0.9$ & $96.7 \pm 0.5$ & $96.4 \pm 0.5$ & $96.5 \pm 0.4$  \\
        \bottomrule
        \bottomrule
    \end{tabular}
}

==> content/13_tables/results_tables/2_ucr-uea-cls-benchmark.tex <==
\adjustbox{max width=\textwidth}{
    %\fontsize{10pt}{12pt}\selectfont
    \begin{tabular}{l|cccccccccccc|c} %cc}
    \toprule
    \toprule
    & \gls{dtwd}\hyperlink{results-footnote}{$^*$} 
    %& \acrshort{dtwi}\hyperlink{results-footnote}{$^*$} 
    & \gls{lstm}\hyperlink{results-footnote}{$^+$} 
    & Rocket\hyperlink{results-footnote}{$^*$} 
    & Mini-Rocket\hyperlink{results-footnote}{$^*$} 
    & \acrshort{tst}\hyperlink{results-footnote}{$^+$} 
    & \acrshort{tst} (pretrained)\hyperlink{results-footnote}{$^+$} 
    & \acrshort{ts2vec}
    & \acrshort{infots} 
    & \acrshort{infots}$_s$ 
    & \acrshort{tarnet}\hyperlink{results-footnote}{$^*$} 
    & \acrshort{vitst}\hyperlink{results-footnote}{$^\dagger$} 
    & \acrshort{timesurl} %& Own & %& Own & Own RM 
    & \textbf{\gls{starformer}} \\
    \midrule
    %Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
    %EigenWorms 
    \acrshort{EW} \cite{brown_eigen_2013} & 0.618 & 
    %- & 
    - & 0.650 & 0.790 & - & - %0.720 
    & 0.847 & 0.733 & 0.748 & 0.420 & \textbf{0.878} & \underline{0.870} %& 0.752 & 0.799 
    & 0.850  \\
    
    %EthanolConcentration 
    \acrshort{EC} \cite{large_ethanol_2018} & 0.323 & 
    %0.304 & 
    0.323 & \underline{0.450} & 0.430 &  0.337 & 0.326 & 0.308 & 0.281 & 0.323 &  0.323 & \textbf{0.456} & 0.304
    % & 0.371 & 0.402 
    & 0.393 \\
    
    %FaceDetection 
    \acrshort{FD} \cite{henson_face_2014} & 0.529 & 
    %- & 
    0.577 & 0.638 & 0.612 & 0.681 & \underline{0.689} & 0.501 & 0.534 & 0.525 &  0.641 & 0.632 & 0.608
    % & 0.687 & 0.673 
    & \textbf{0.697}  \\
    
    %Handwriting (
    \acrshort{HW} \cite{shokoohi-yekta_handwriting_2017} & 0.286 & 
    %0.316 & 
    0.152 & \textbf{0.596} & 0.520 & 0.305 & 0.359 & 0.515 & 0.452 & \underline{0.554} & 0.281 & - & 0.462
    % & 0.336 & 0.327 
    & 0.373   \\
    
    % Heartbeat (
    \acrshort{HB} \cite{goldberger_heartbeat_2016} & 0.717 & %0.658 & 
    0.722 & 0.741 & 0.771 & \underline{0.776} & \underline{0.776} & 0.683 & 0.722 & 0.771 & \textbf{0.780} & 0.766 & 0.746
    %& \textbf{0.786} & 0.772 
    & 0.772  \\

    %JapaneseVowels (
    \acrshort{JV} \cite{kudo_japanese_1999} & 0.949 & %0.959 & 
    0.797 & 0.978 & 0.986 & \underline{0.994} & \textbf{0.997} & 0.984 & 0.984 & 0.986 &  0.992 & 0.946 & 0.989
    %& 0.989 & 0.982 
    & 0.990 \\
    
    %PenDigits (
    \acrshort{PD} \cite{alimoglu_pen_1996} & 0.977 & 0.939 & %- & 
    0.981 & 0.967 & - & %\underline{0.981} 
    - & \underline{0.989} & \textbf{0.990} & \underline{0.989} &  0.976 & - & \underline{0.989}
    %& \textbf{0.982} & 0.980 
    & 0.983  \\
    
    %PEMS-SF (
    \acrshort{PS} \cite{cuturi_pems-sf_2009} & 0.711 & % 0.734 & 
    0.399 & 0.832 & 0.809 & 0.919 & 0.896 & 0.682 & 0.751 & 0.757 &  \underline{0.936} & 0.913 & 0.821
    %& 0.841 & 0.922 
    & \textbf{0.943}  \\
    
    % SelfRegulationSCP1 (
    \acrshort{SCP1} \cite{hinterberger_self_1999-1} & 0.775 & % 0.765 &
    0.689 & 0.867 & 0.915 & \textbf{0.925} & \underline{0.922} & 0.812 & 0.874 & 0.887 & 0.816 & 0.898 & 0.908 %& 0.906 & 0.891 
    & 0.913 \\

    % SelfRegulationSCP2 (
    \acrshort{SCP2} \cite{hinterberger_self_1999} & 0.539 & %0.533 &
    0.466 & 0.555 & 0.506 & 0.589 & 0.604 & 0.578 & 0.578 & 0.572 & \underline{0.622} & 0.561 & 0.600
    %& 0.630 & 0.620 
    & \textbf{0.635} \\

    %SpokenArabicDigits (
    \acrshort{SAD} \cite{hammami_spoken_2010} & 0.963 & %0.959	
    0.319 & 0.997 & 0.963 & \underline{0.993} & \textbf{0.998} & 0.988 & 0.947 & 0.932 & 0.985 & 0.985 & 0.985
    %& 0.990 & 0.983 
    & 0.989 \\
    
    %UWaveGestureLibrary (
    \acrshort{UW} \cite{liu_u_2009} & 0.903 & %0.868 & 
    0.412 & \textbf{0.931} & 0.785 & 0.903 & \underline{0.913} & 0.906 & 0.884 & 0.884 & 0.878 & 0.862 & 0.919
    %& 0.881 & 0.838 
    & 0.894 \\
    
    \midrule
    %Average Accuracy & 0.691 & 0.706 & 0.486 & 0.768 & 	0.755 & 0.742 & 0.765 & 0.721 & \textbf{0.790} 
    %& 0.768 & 0.766 
    %& \underline{0.784}  \\
    %Rank & 9 & 8 & 10 & 3 & 5 & 6 & 4 & 7 & \textbf{1} 
    %& - & - 
    %& \underline{2} \\
    %Average Rank & 7.0 & 8.0 & 6.2 & 4.1 & 5.5 & 3.2 & \textbf{2.8} & 4.8 & 4.9 
    %& - & - 
    %& \underline{2.9}  \\
    %Num. of Top Scores & 0 & 0 & 0 & 2 %& 0 & 1 & 3 & 1 & 2 
    % & - & -
    %& \textbf{4} \\
    %STaR-ADReM 1-v-1& 11 & 10 & 10 & 8 & 9 & 9 & 7 & 10 & 7 
    %& 7 & 10 
    %& -  \\
    %Dataset Count & 12 & 10 & 10 & 12 & 12 & 10 & 12 & 12 & 10 
    %& 12 & 12 
    %& 12 \\
    %\midrule
    %%%%%%% Average 8 %%%%%%% 
    %Average Accuracy 8 & 0.735 & 0.723 & 0.516 & 0.794 & 0.771 & \underline{0.805} & 0.804 & 0.743 & 0.753 & 0.764 & 0.792 & 0.798 & \textbf{0.816} \\
    %Rank 8 & 11 & 12 & 13 & 5 & 7 & \underline{2} & 3 & 10 & 9 & 8 & 6 & 4
    %& \underline{2} & 5 
    %& \textbf{1} \\
    %Average Rank 8 & 9.1 & 11.0 & 11.8 & 5.6 & 6.9 & \underline{3.0} & \textbf{2.8} & 8.1 & 8.5 & 7.1 & 4.9 & 6.8
    %& 4.1 & 6.0 
    %& 3.5 \\
    %Num. of Top Scores & 0 & 0 & 0 & 2 & 0 & 1 & 2 & 0 & 1 & 0 & 1 & 2 
    % & - & -
    %& \textbf{3} \\
    %STaRFormer 1-v-1 & 11 & 10 & 10 & 8 & 9 & 5 & 6 & 9 & 10 & 10 & 10 & 8 & -\\
    %Dataset Count & 12 & 10 & 10 & 12 & 12 & 10 & 10 & 12 & 12 & 12 & 12 & 10 
    %& 12 & 12 
    %& 12 \\
    %%%%%%% Average 9 %%%%%%%
    Average Accuracy 9 & 0.712 & 0.523 & 0.777 & 0.753 & 0.790 & \underline{0.791} & 0.716 & 0.728 & 0.737 & 0.775 & 0.780 & 0.764 & \textbf{0.803} \\
    Rank 9 & 12 & 13 & 5 & 8 & 3 & \underline{2} & 11 & 10 & 9 & 6 & 4 & 7 & \textbf{1} \\
    Average Rank 9 & 10.1 &	12.2 & 6.0 & 7.4 & \underline{3.2} & \textbf{2.8} & 9.3 & 9.6 & 8.3 & 5.0 & 7.1 & 6.3 & 3.3 \\
    Num. of Top Scores & 0 & 0 & 2 & 0 & 1 & 2 & 0 & 1 & 0 & 1 & 2 & 0 
    & \textbf{3} \\
    STaRFormer 1-v-1 & 11 & 10 & 8 & 9 & 5 & 5 & 9 & 10 & 10 & 10 & 8 & 8 & -\\
    Dataset Count & 12 & 10 & 12 & 12 & 10 & 10 & 12 & 12 & 12 & 12 & 10 & 12 & 12\\ 
    \bottomrule
    \bottomrule
    \end{tabular}
}
